The Impact of Generative Artificial Intelligence on Market Equilibrium: Evidence from a Natural Experiment

Generative artificial intelligence (AI) exhibits the capability to generate creative content akin to human output with greater efficiency and reduced costs. This groundbreaking capability, however, has ignited a debate regarding its potential to displace human creators. In light of these discussions, this paper empirically investigates the impact of generative AI on market equilibrium, in the context of China's leading art outsourcing platform. We overcome the challenge of causal inference by identifying an unanticipated and sudden leak of an advanced image-generative AI as a natural experiment. This leak precipitated a notable reduction in the production costs of anime-style images compared to other genres, thereby providing a unique opportunity for difference-in-differences comparisons. Our analysis shows that the advent of generative AI led to a 64% reduction in average prices, yet it simultaneously spurred a 121% increase in order volume and a 56% increase in overall revenue. This growth is primarily driven by the rising demand for "low-end" personal orders, rather than commercial orders. Moreover, incumbent creators retain the majority of the market share and reap the most benefits of generative AI. Our research highlights the potential of generative AI to benefit all stakeholders across the platform economy, yielding both scholarly contributions and practical implications.

==> sections/00.rebuttal.tex <==
\newpage
\subsection{Q1: Why are this paper's findings significant?}
The economic theory suggests that generative AI could result in either (1) a decrease in both price and volume or (2) a decrease in price but an increase in volume. \textbf{While the two potential outcomes may seem trivial in isolation, we did not know which outcome reflects reality.} Will painter jobs disappear like translator jobs? This paper demonstrates that the more favorable of the two outcomes represents reality: the number of orders rises by as much as 121\%, and total revenue grows by 54\% despite a 67\% drop in average price.

Admittedly, AI scientists would be optimistic about the impact of generative AI, believing that their work will make the world a better place. Conversely, sectors of the general public, such as artists, often express negative views, as evidenced by various protests. The findings of this paper can tell them what was considered harmful is actually beneficial and that the benefits are indeed substantial. As such, it is fair to say that the findings of this study are surprising.

\subsection{Q2: How does this paper contribute to AAAI?}
Recently, there has been a debate about the regulatory framework for generative AI. Turing Award Laureates Geoffrey Hinton and Yoshua Bengio argue for strict regulation because of the "risk of extinction by AI". Conversely, Yann LeCun takes the opposite view, arguing that strict regulation could hinder the development of generative AI. Which perspective should a policymaker on generative AI support? 

To make an informed decision, the policymaker might seek empirical evidence to determine, whether generative AI creates or eliminates more jobs, whether it generates more or less tax revenue, and so on. In this context, research papers that focus on the development of new algorithms may not provide the necessary insights. Therefore, this paper aims to make an economic rather than a technical contribution by presenting empirical evidence to address these pertinent questions that are closely related to the AI community.

\subsection{Response to Reviewer \#1}
Thanks for your reviews. Please refer to sections Q1 and Q2. 

In addition, I argue that the analysis in this paper is non-trivial due to the well-identified natural experiment, which overcomes the difficulty of causal inference. This is analogous to the anecdote involving the Ford Company and Charles Steinmetz, in which \textbf{making the mark itself was worth only \$1, while understanding where to make a chalk mark was valued at \$9,999}.
% Moreover, the application of the identified natural experiment extends beyond the study of its impact on product markets. For example, its application to LinkedIn data could facilitate a comprehensive study of the impact of generative AI on labor markets.
\subsection{Response to Reviewer \#2}
Thank you for your reviews. I'm glad to receive appreciation and critiques from an expert in economics.

\textbf{W1}: The use of a short window serves to emphasize the natural experiment and reduce the risk of confounding factors. In addition, I also extended the window to one year, ending last month. The resulting percentage changes in price, volume, and turnover are -69\%, 154\%, and 85\%, respectively, further supporting the arguments in this study.

This paper is not intended to fully answer the very broad question of how generative AI will affect creative workers in a single paper. However, this paper contributes to answering this question by providing empirical evidence that artists have more orders and income from product markets. Moreover, the identified natural experiment facilitates follow-up research beyond product markets. For example, its application to LinkedIn data could answer the question of how generative AI will affect creative workers in labor markets.

\textbf{W2}: Please refer to section Q1.

\textbf{W3}: It depends on how we define artists. Artists in the past used canvas and paint; artists today use digital boards and Photoshop. It is totally fine for artists of the future to use generative AI. 
To further address your concern, I conducted a heterogeneous analysis for incumbent artists, who registered before the leak. Counting only the orders completed by incumbents, I find that incumbents receive 155\% more orders and 84\% more turnover, with a 71\% decrease in average price. In fact, incumbents take 97.4\% of orders and 98\% of turnover for all orders after the leak. 
% This is also another piece of evidence that answers how generative AI will affect creative workers.

\subsection{Response to Reviewer \#3}
Thank you for your humble reviews and open questions.

% Given that generative AI has been invented, the introduction of AI into workflows can of course increase the efficiency of artists now. 
In the future, if human-quality images can be generated automatically, this could theoretically lead to a decrease in the demand for artists. If demand were to drop to zero, then being an artist could not be a job. But from my observations, I don't think that will be the case, because artists also serve a communication role, given that many clients cannot articulate exactly what they want.
\subsection{Response to Reviewer \#4}
Thanks for your reviews, although it's inappropriate to judge an economics paper by the metrics of algorithm papers.

\textbf{W1}: First, the general public is unlikely to be able to implement AI. They may not even know about Github or Stable Diffusion. Second, Chinese is difficult to access these resources due to political and language reasons. Third, the search engine index in China (Baidu Index) on "AI drawing" or "stable diffusion" can address your concern, which surged from 0 to above, just around the leak.

Novelai leaked their trained models more than codes. The potential outcome framework, which won the Nobel Prize in 2021, can infer the correct causal impact without being affected by the "many factors" you mentioned.

\textbf{W2}: The change is for tachie, not wallpaper market.

\textbf{W3, W4}: Most economic papers, including those published in Nature/Science or with thousands of citations, use one dataset to justify their claims. They generalize their findings through theories, as informed in Figure 4 for this paper.

\textbf{W5}: The natural experiment in this paper allows the study of the impact of generative AI beyond the market equilibrium studied in this paper. Like the Transformer paper, it studies only the English-to-German translation task, but its attention structure can be applied in many places.

\textbf{W6}: Figure 1 informs readers that artists think they are suffering from generative AI, although generative AI is not as bad as they thought. Figure 3 informs readers about the type and quality of images the leaked model can generate. It supports why the leak only affects the tachie market and not the wallpaper market.

\newpage

==> sections/6.explain.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1\textwidth]{images/supply.png}
  \caption{Theoretical Explanations for the Impact of Generative AI on Market Equilibrium}
  \label{fig:supply}
  % \vspace{-5mm}
\end{figure*}

\section{Theoretical Explanation}
In this section, we elucidate and generalize our findings presented in Section~\ref{sec:main} through the lens of market equilibrium theory in microeconomics.

The market equilibrium theory explains how prices and quantities of goods and services are determined in a market, as shown in Figure~\ref{fig:supply}(a). The theory is based on the interaction between two key forces: supply and demand. Supply refers to the quantity of a good that producers are willing to offer for sale at different price levels. Demand represents the willingness of consumers to purchase a certain quantity of a good at various price levels. The relationship between price and quantity supplied is depicted on a supply curve, which slopes upward from left to right; the relationship between price and quantity demanded is illustrated on a demand curve, which slopes downward from left to right.

The equilibrium price and quantity in a market are determined by the intersection of the demand and supply curves. This point is known as the market equilibrium. The equilibrium in Figure~\ref{fig:supply}(a) is $(Q_0,P_0)$, which represents the market equilibrium before generative AI.
% The supply and demand model explains how prices and quantities of goods and services are determined in a market, as shown in Figure~\ref{fig:supply}(a). It revolves around the interaction between two key forces: supply and demand. 

% Demand represents the willingness and ability of consumers to purchase a certain quantity of a good or service at various price levels. All else being equal, as the price of a good or service decreases, the quantity demanded increases, and vice versa. This inverse relationship between price and quantity demanded is often illustrated on a demand curve, which slopes downward from left to right.

% Supply refers to the quantity of a good or service that producers are willing and able to offer for sale at different price levels. All else being equal, as the price of a good or service increases, the quantity supplied also increases. This positive relationship between price and quantity supplied is often depicted on a supply curve, which slopes upward from left to right.

% The equilibrium price and quantity in a market are determined by the intersection of the demand and supply curves. This point is known as the market equilibrium. The equilibrium in Figure~\ref{fig:supply}(a) is $(Q_0,P_0)$, which represents the market equilibrium before generative AI.

We show that Generative AI can shift the demand curve inward and the supply curve outward.

Consumers might prefer AI-generated content over real-world alternatives because they are cheaper, more convenient, and customizable. As a result, these AI-generated alternatives are close substitutes for real-world products, which might reduce consumer demand for the actual products and lead to a shift in the demand curve inward (Figure~\ref{fig:supply}(b)). In contrast, generative AI can also increase productivity for producers. For example, artists can employ generative AI to initially generate an image at 80\% quality and then refine the generated output to achieve 100\% quality. The increased productivity can lead to increased supply as producers are able to produce more output within the same amount of time and effort, shifting the demand curve outward (Figure~\ref{fig:supply}(c)).

Shifting the demand curve inward reduces the equilibrium price and quantity. Shifting the supply curve outward reduces the price but increases the quantity. Generative AI can shift both the demand curve inward and the supply curve outward, which has two possible equilibria: in Figure~\ref{fig:supply}(d), both price and quantity decrease ($P_1<P_0,Q_1<Q_0$) relative to the initial equilibrium; in Figure~\ref{fig:supply}(e), price decreases but quantity increases ($P_2<P_0,Q_2>Q_0$).

The market equilibrium theory indicates two possible equilibria for the impact of generative AI. Our empirical results provide evidence that its impact belongs to the more promising outcome, Figure~\ref{fig:supply}(e), of the two. Moreover, our empirical results further show that overall revenue ($PQ$) also increases, which is uncertain according to the theory.





==> sections/7.implication.tex <==
\section{Implications}
The counterintuitive findings in this paper have significant implications for various stakeholders.

\textbf{Practitioners}. The most direct implication for practitioners is that they should welcome generative AI instead of resisting it, because generative AI can increase their income and make their industry more prosperous. As economic theory suggests, generative AI helps them by increasing their efficiency. As a result, practitioners should think about how to incorporate generative AI into their workflow to improve it. For example, in the past, artists completed a painting by sketching, line drawing, and coloring. They can use generative AI to get a base and "fine tune" it in the future.

\textbf{Policymakers}. Although generative AI has other issues, such as intellectual property concerns, policy making is a comprehensive consideration. This paper provides empirical evidence in favor of generative AI in that it can increase taxes and contribute to upstream and downstream markets by increasing the number of orders and total revenue. On the other hand, a misunderstanding of the economic consequences of generative AI may lead to a wrong policy, causing the country to miss out on the new wave of development brought by AI.

\textbf{AI community}. When the concept of artificial intelligence was born, so were the fears that AI could destroy human society. In the movie The Terminator, the AI system invented by computer scientists ultimately caused the end of the world. In addition to lobbying for more investment in the AI community, this article can, more importantly, assuage any unease and guilt that researchers may feel because the empirical evidence in the article shows that generative AI is augmenting humans rather than replacing them.

==> sections/alter_price_table.tex <==
\begin{table*}[h!]
% \linespread{1}
% \huge
% \selectfont
% \footnotesize
\centering
    % \vspace{-5mm}
    \resizebox{\linewidth}{!}{
   \begin{tabular}{lcccccccc}
      \tabularnewline \midrule \midrule

      Dependent Variables:    & log(price\_upper)        & log(revenue\_upper)      & log(price\_middle)       & log(revenue\_middle)  & log(price\_ul)           & log(revenue\_ul)         & log(price\_lu)           & log(revenue\_lu)\\   
      Model:                  & (1)                      & (2)                      & (3)                      & (4)                   & (5)                      & (6)                      & (7)                      & (8)\\  
      \midrule
      \emph{Variables}\\
      treated $\times$ after  & -0.5168$^{***}$          & 0.6940$^{***}$           & -0.5564$^{***}$          & 0.6544$^{***}$        & -0.3046$^{***}$          & 0.9062$^{***}$           & -0.8558$^{***}$          & 0.3549$^{***}$\\   
                              & ($1.71\times 10^{-15}$)  & ($1.39\times 10^{-15}$)  & ($1.43\times 10^{-15}$)  & ($2\times 10^{-15}$)  & ($7.52\times 10^{-16}$)  & ($2.74\times 10^{-15}$)  & ($2.16\times 10^{-15}$)  & ($1.35\times 10^{-15}$)\\    
      \midrule
      \emph{Fixed-effects}\\
      art\_category           & Yes                      & Yes                      & Yes                      & Yes                   & Yes                      & Yes                      & Yes                      & Yes\\  
      year\_week              & Yes                      & Yes                      & Yes                      & Yes                   & Yes                      & Yes                      & Yes                      & Yes\\  
      \midrule
      \emph{Fit statistics}\\
      Observations            & 126                      & 126                      & 126                      & 126                   & 126                      & 126                      & 126                      & 126\\  
      R$^2$                   & 0.84131                  & 0.84148                  & 0.87004                  & 0.85222               & 0.95451                  & 0.92018                  & 0.95013                  & 0.94098\\  
      Within R$^2$            & 0.42816                  & 0.44333                  & 0.47405                  & 0.42184               & 0.20118                  & 0.58389                  & 0.67316                  & 0.17232\\  
      \midrule \midrule
      \multicolumn{9}{l}{\emph{Clustered (art\_category) standard-errors in parentheses}}\\
      \multicolumn{9}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\



   \end{tabular}  
   }

% \vspace{+5mm}
\caption{The Impact of Generative AI on Market Equilibrium - Alternative Price Measurements}
\label{tab:reg_alterprice}
\end{table*}

==> sections/completed_table.tex <==
\begin{table*}[!t]
% \linespread{1}
% \huge
% \selectfont
% \footnotesize
\centering
    % \vspace{-5mm}
    \resizebox{\linewidth}{!}{
   \begin{tabular}{lcccccc}
      \tabularnewline \midrule \midrule
      Dependent Variables:    & price                    & volume                   & revenue                 & log(price)               & log(volume)              & log(revenue)\\  
      Model:                  & (1)                      & (2)                      & (3)                      & (4)                      & (5)                      & (6)\\  
      \midrule
      \emph{Variables}\\
      treated $\times$ after  & -502.4$^{***}$           & 45.77$^{***}$            & 23,375.2$^{***}$         & -0.4915$^{***}$          & 1.171$^{***}$            & 0.6790$^{***}$\\   
                              & ($1.59\times 10^{-12}$)  & ($1.17\times 10^{-13}$)  & ($7.54\times 10^{-11}$)  & ($1.33\times 10^{-15}$)  & ($3.51\times 10^{-15}$)  & ($2.02\times 10^{-15}$)\\    
      \midrule
      \emph{Fixed-effects}\\
      art\_category           & Yes                      & Yes                      & Yes                      & Yes                      & Yes                      & Yes\\  
      year\_week              & Yes                      & Yes                      & Yes                      & Yes                      & Yes                      & Yes\\  
      \midrule
      \emph{Fit statistics}\\
      Observations            & 126                      & 126                      & 126                      & 126                      & 126                      & 126\\  
      R$^2$                   & 0.77403                  & 0.85943                  & 0.73179                  & 0.79706                  & 0.89378                  & 0.73652\\  
      Within R$^2$            & 0.22630                  & 0.72652                  & 0.24330                  & 0.21484                  & 0.67848                  & 0.19868\\  
      \midrule \midrule
      \multicolumn{7}{l}{\emph{Clustered (art\_category) standard-errors in parentheses}}\\
      \multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

   \end{tabular}  
   }

% \vspace{+5mm}
\caption{The Impact of Generative AI on Market Equilibrium - Completed Order Results}
\label{tab:completed}
\end{table*}

==> sections/longer_table.tex <==
\begin{table*}[h!]
% \linespread{1}
% \huge
% \selectfont
% \footnotesize
\centering
    % \vspace{-5mm}
    \resizebox{\linewidth}{!}{
   \begin{tabular}{lcccccc}
      \tabularnewline \midrule \midrule
      Dependent Variables:    & price                    & volume                   & revenue                 & log(price)               & log(volume)              & log(revenue)\\  
      Model:                  & (1)                      & (2)                      & (3)                      & (4)                      & (5)                      & (6)\\  
      \midrule
      \emph{Variables}\\
      treated $\times$ after  & -772.9$^{***}$           & 177.1$^{***}$            & 56,384.1$^{***}$         & -0.8181$^{***}$          & 1.550$^{***}$            & 0.7318$^{***}$\\   
                              & ($5.14\times 10^{-12}$)  & ($1.17\times 10^{-12}$)  & ($3.87\times 10^{-10}$)  & ($5.14\times 10^{-15}$)  & ($8.55\times 10^{-15}$)  & ($4.62\times 10^{-15}$)\\    
      \midrule
      \emph{Fixed-effects}\\
      art\_category           & Yes                      & Yes                      & Yes                      & Yes                      & Yes                      & Yes\\  
      year\_week              & Yes                      & Yes                      & Yes                      & Yes                      & Yes                      & Yes\\  
      \midrule
      \emph{Fit statistics}\\
      Observations            & 186                      & 186                      & 186                      & 186                      & 186                      & 186\\  
      R$^2$                   & 0.86955                  & 0.88528                  & 0.87977                  & 0.87633                  & 0.89432                  & 0.89620\\  
      Within R$^2$            & 0.63660                  & 0.82983                  & 0.43064                  & 0.63307                  & 0.83147                  & 0.48623\\  
      \midrule \midrule
      \multicolumn{7}{l}{\emph{Clustered (art\_category) standard-errors in parentheses}}\\
      \multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

   \end{tabular}  
   }

% \vspace{+5mm}
\caption{The Impact of Generative AI on Market Equilibrium - Longer Time Period}
\label{tab:longer}
\end{table*}

==> sections/placebo_table.tex <==
\begin{table*}[h!]
% \linespread{1}
% \huge
% \selectfont
% \footnotesize
\centering
    % \vspace{-5mm}
    \resizebox{\linewidth}{!}{
   \begin{tabular}{lcccccc}
      \tabularnewline \midrule \midrule
      Dependent Variables:    & price                 & volume   & revenue & log(price)            & log(volume)  & log(revenue)\\  
      Model:                  & (1)                   & (2)      & (3)     & (4)                   & (5)          & (6)\\  
      \midrule
      \emph{Variables}\\
      treated $\times$ after  & -22.62                & 0.5474   & 399.3   & -0.0112               & 0.1311$^{*}$ & 0.1199\\   
                              & (106.7)               & (0.5632) & (910.9) & (0.0740)              & (0.0688)     & (0.1055)\\   
      \midrule
      \emph{Fixed-effects}\\
      art\_category           & Yes                   & Yes      & Yes     & Yes                   & Yes          & Yes\\  
      year\_week              & Yes                   & Yes      & Yes     & Yes                   & Yes          & Yes\\  
      \midrule
      \emph{Fit statistics}\\
      Observations            & 716                   & 716      & 716     & 716                   & 716          & 716\\  
      R$^2$                   & 0.41401               & 0.63994  & 0.22616 & 0.55645               & 0.61816      & 0.30111\\  
      Within R$^2$            & $7.75\times 10^{-5}$  & 0.00186  & 0.00034 & $3.32\times 10^{-5}$  & 0.00726      & 0.00227\\  
      \midrule \midrule
      \multicolumn{7}{l}{\emph{Clustered (lastdigit) standard-errors in parentheses}}\\
      \multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

   \end{tabular}  
   }

% \vspace{+5mm}
\caption{The Impact of Generative AI on Market Equilibrium - Placebo Test}
\label{tab:placebo_fake}
\end{table*}


\begin{table*}[h!]
% \linespread{1}
% \huge
% \selectfont
% \footnotesize
\centering
    % \vspace{-5mm}
    \resizebox{\linewidth}{!}{
   \begin{tabular}{lcccccc}
      \tabularnewline \midrule \midrule
      Dependent Variables:    & price          & volume        & revenue         & log(price)      & log(volume)   & log(revenue)\\  
      Model:                  & (1)            & (2)           & (3)             & (4)             & (5)           & (6)\\  
      \midrule
      \emph{Variables}\\
      treated $\times$ after  & -656.6$^{***}$ & 14.06$^{***}$ & 5,702.6$^{***}$ & -0.5630$^{***}$ & 1.249$^{***}$ & 0.6864$^{***}$\\   
                              & (48.88)        & (0.3398)      & (654.3)         & (0.0507)        & (0.0412)      & (0.0692)\\   
      \midrule
      \emph{Fixed-effects}\\
      art\_category           & Yes            & Yes           & Yes             & Yes             & Yes           & Yes\\  
      year\_week              & Yes            & Yes           & Yes             & Yes             & Yes           & Yes\\  
      \midrule
      \emph{Fit statistics}\\
      Observations            & 1,253          & 1,253         & 1,253           & 1,253           & 1,253         & 1,253\\  
      R$^2$                   & 0.41023        & 0.65433       & 0.34534         & 0.48933         & 0.66103       & 0.39564\\  
      Within R$^2$            & 0.08167        & 0.45615       & 0.05610         & 0.07988         & 0.41087       & 0.07020\\  
      \midrule \midrule
      \multicolumn{7}{l}{\emph{Clustered (lastdigit) standard-errors in parentheses}}\\
      \multicolumn{7}{l}{\emph{Signif. Codes: ***: 0.01, **: 0.05, *: 0.1}}\\

   \end{tabular}  
   }

% \vspace{+5mm}
\caption{The Impact of Generative AI on Market Equilibrium - Real Treatment Date}
\label{tab:placebo_real}
\end{table*}
